A Survey of DevOps Concepts and Challenges

DevOps is a collaborative and multidisciplinary organizational effort to automate continuous delivery of new software updates while guaranteeing their correctness and reliability. The present survey investigates and discusses DevOps challenges from the perspective of engineers, managers, and researchers. We review the literature and develop a DevOps conceptual map, correlating the DevOps automation tools with these concepts. We then discuss their practical implications for engineers, managers, and researchers. Finally, we critically explore some of the most relevant DevOps challenges reported by the literature.

==> tabs/tab-research-challenges.tex <==
{
\small

\begin{table}[ht]
\centering
\caption{Research challenges on \devops}
\label{tab:research-challenges}
\begin{tabular}{l} \hline
Architecturing in the \devops context\\
\devops training\\
\devops and embedded systems\\
\devops and compliance\\
\devops and security\\
Testing large-scale distributed systems\\
Ever-changing \devops tools\\
Metrics usage in research on \devops\\
Improving interdepartmental communication\\
\devops adoption strategies\\
\hline
\end{tabular}
\end{table}

% end small
}

